Robust Accent Identification via Voice Conversion and Non-Timbral Embeddings

Automatic accent identification (AID) remains a challenging task due to the complex variability of accents, the entanglement of accent cues with speaker traits, and the scarcity of reliable accentlabelled data. To address these challenges, we propose a speaker augmentation strategy using voice conversion (VC), with which we generate additional training data by converting original training utterances into different speaker voices while preserving accentual cues. For this purpose, we select two recent VC systems and evaluate their capability to preserve accent. Alternatively, we also explore the use of non-timbral embeddings in AID, for their ability to convey accent information among other non timbral cues. The effectiveness of both methods is demonstrated on the GenAID benchmark, achieving a new state-of-the-art F1-score of 0.66, compared to the previous score of 0.55. Beyond AID, we show that non-timbral embeddings enable accent-controlled Text-to-Speech, producing high-fidelity speech with accurate accent transfer.

==> rebutall.tex <==

Rebutall  for paper title:  ROBUST ACCENT IDENTIFICATION VIA VOICE CONVERSION AND NON-TIMBRAL EMBEDDINGS

% We thank all the reviewers for their careful evaluation, constructive feedback, and the positive comments about the relevance and clarity of our work. Below, we clarify points raised by the reviewers.

% While 7EB9 highlights several important strengths, concerns are raised regarding limited methodological novelty. We respectfully disagree with this characterisation. This work does not primarily aim to introduce a new model architecture, but rather to provide the first systematic analysis of voice conversion (VC) behaviour for designing speaker-augmentation strategies in accent identification, combined with the use of non-timbral embeddings. Using GenAID as a strong state-of-the-art baseline, we demonstrate a clear and substantial improvement of 11 points on F1 in unseen-speaker performance, which multiple reviewers acknowledge as significant. This statement also answers the request from 4615 for a clear comparison with existing accent-classification.

% Reviewer 3438 recognises the overall quality but raises concerns that allegedly undermine the paper's claim, which we address and refute throughout the rest of this rebuttal. While we agree that additional side experiments could be added, we clarify that the task studied is accent identification (AID) - legitimately evaluated via classifier performance and accent-embedding cosine similarity - not perceptual accent assessment. Our goal is to analyse whether accent-related information, as exploited by machine classifiers, is preserved under VC while speaker timbre is altered : human perceptual evaluations are beyond the scope of this work.

% Questions regarding the number of VC augmentations and combinations of VC methods are already addressed in Section 6 (third paragraph). We have demonstrated that combining both RVC- and kNN-VC–generated data did not yield additional gains. This result motivated our final configuration and suggests that increasing augmentation diversity is unnecessary in this setting.

% While stronger classifiers and additional ablations could be explored, they do not undermine the main finding. Under a controlled and consistent setup, VC-based augmentation and non-timbral embeddings yield robust and significant improvements in unseen-speaker AID from 0.55 to 0.66 F1-score. The adversarial speaker head follows the GenAID setup to ensure fair comparison and further encourages accent-consistent representations.

% Finally, the TTS evaluation outputs using the same GenAID classifier should be beneficial for WTA+GenAID, in Table 3 which is already discussed in the second paragraph of Section 7. On the contrary, this enhances the relevance and effectiveness of using our WTA+WNTA setting. The reviewer appears to have misunderstood this point.




%Nick version
=====
We are delighted with the predominantly positive and constructive feedback. 

We respectfully disagree with reviewer 7EB9 about the alleged limited novelty of our work, as we propose a method that significantly improves accent classification performance: using GenAID as a strong state-of-the-art baseline, we show a clear comparison with existing accent-classification and demonstrate a substantial improvement of 11 points on F1 in unseen-speaker performance, which multiple reviewers acknowledge as significant. 

While more additional side experiments could be always added, we believe that those proposed by reviewer 3438 are unnecessary and irrelevant. The task studied is accent identification (AID) - legitimately evaluated via classifier performance and accent-embedding cosine similarity - not perceptual accent assessment. Our goal is to analyse whether accent-related information, as exploited by machine classifiers, is preserved under VC while speaker timbre is altered : human perceptual evaluations are beyond the scope of this work. 

Similarly, while alternative classifiers and additional ablations can always be explored, they would not affect our conclusions: under a controlled and consistent setup, VC-based augmentation and non-timbral embeddings yield robust and significant improvements in unseen-speaker AID from 0.55 to 0.66 F1-score. The adversarial speaker head follows the GenAID setup to ensure fair comparison and further encourages accent-consistent representations.

Finally, the TTS evaluation outputs using the same GenAID classifier should be beneficial for WTA+GenAID, in Table 3 which is already discussed in the second paragraph of Section 7. On the contrary, this enhances the relevance and effectiveness of using our WTA+WNTA setting. The reviewer appears to have misunderstood this point.



